A Formalization of the Ionescu-Tulcea Theorem in Mathlib

We describe the formalization of the Ionescu-Tulcea theorem, showing the existence of a probability measure on the space of trajectories of a Markov chain, in the proof assistant Lean using the integrated library Mathlib. We first present a mathematical proof before exposing the difficulties which arise when trying to formalize it, and how they were overcome. We then build on this work to formalize the construction of the product of an arbitrary family of probability measures.

==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

	% Anything between $ becomes LaTeX math mode
	mathescape=false,
	% Comments may or not include Latex commands
	texcl=false,

	% keywords, list taken from lean-syntax.el
	morekeywords=[1]{
		import, prelude, protected, private, noncomputable, definition, meta, renaming,
		hiding, parameter, parameters, begin, constant, constants,
		lemma, variable, variables, theory,
		print, theorem, example,
		open, as, export, override, axiom, axioms, inductive, with,
		structure, record, universe, universes,
		alias, help, precedence, reserve, declare_trace, add_key_equivalence,
		match, infix, infixl, infixr, notation, postfix, prefix, instance,
		eval, reduce, check, end, this,
		using, using_well_founded, namespace, section,
		attribute, local, set_option, extends, include, omit, class,
		raw, replacing,
		calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
		exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
		mutual, do, def, run_cmd, const,
		partial, mut, where, macro, syntax, deriving,
		return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

	% Sorts
	morekeywords=[2]{Sort, Type, Prop},

	% tactics, list taken from lean-syntax.el
	morekeywords=[3]{
		assumption,
		apply, intro, intros, allGoals,
		generalize, clear, revert, done, exact,
		refine, repeat, cases, rewrite, rw,
		simp, simp_all, contradiction,
		constructor, injection,
		induction,
	},

	% modifiers, taken from lean-syntax.el
	% note: 'otherkeywords' is needed because these use a different symbol.
	% this command doesn't allow us to specify a number -- they are put with [1]
	% otherkeywords={
		% [persistent], [notation], [visible], [instance], [trans_instance],
		% [class], [parsing-only], [coercion], [unfold_full], [constructor],
		% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
		% [whnf], [multiple_instances], [none], [decl], [declaration],
		% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
		% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
		% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
		% [localrefinfo], [recursor]
		% },

	% Various symbols
	literate=
	{α}{{\ensuremath{\mathrm{\alpha}}}}1
	{β}{{\ensuremath{\mathrm{\beta}}}}1
	{γ}{{\ensuremath{\mathrm{\gamma}}}}1
	{δ}{{\ensuremath{\mathrm{\delta}}}}1
	{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
	{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
	{η}{{\ensuremath{\mathrm{\eta}}}}1
	{θ}{{\ensuremath{\mathrm{\theta}}}}1
	{ι}{{\ensuremath{\mathrm{\iota}}}}1
	{κ}{{\ensuremath{\mathrm{\kappa}}}}1
	{μ}{{\ensuremath{\mathrm{\mu}}}}1
	{ν}{{\ensuremath{\mathrm{\nu}}}}1
	{ξ}{{\ensuremath{\mathrm{\xi}}}}1
	{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
	{ρ}{{\ensuremath{\mathrm{\rho}}}}1
	{σ}{{\ensuremath{\mathrm{\sigma}}}}1
	{τ}{{\ensuremath{\mathrm{\tau}}}}1
	{φ}{{\ensuremath{\mathrm{\varphi}}}}1
	{χ}{{\ensuremath{\mathrm{\chi}}}}1
	{ψ}{{\ensuremath{\mathrm{\psi}}}}1
	{ω}{{\ensuremath{\mathrm{\omega}}}}1

	{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
	{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
	{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
	{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
	{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
	{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
	{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
	{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
	{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

	{ℵ}{{\ensuremath{\aleph}}}1

	{≤}{{\ensuremath{\leq}}}1
	{≥}{{\ensuremath{\geq}}}1
	{≠}{{\ensuremath{\neq}}}1
	{≈}{{\ensuremath{\approx}}}1
	{≡}{{\ensuremath{\equiv}}}1
	{≃}{{\ensuremath{\simeq}}}1

	{≤}{{\ensuremath{\leq}}}1
	{≥}{{\ensuremath{\geq}}}1

	{∂}{{\ensuremath{\partial}}}1
	{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

	{∫}{{\ensuremath{\int}}}1
	{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
	{Π}{{\ensuremath{\mathrm{\Pi}}}}1
	{Π}{{\ensuremath{\mathrm{\Pi}}}}1

	{⊥}{{\ensuremath{\perp}}}1
	{∞}{{\ensuremath{\infty}}}1
	{∂}{{\ensuremath{\partial}}}1

	{∓}{{\ensuremath{\mp}}}1
	{±}{{\ensuremath{\pm}}}1
	{×}{{\ensuremath{\times}}}1

	{⊕}{{\ensuremath{\oplus}}}1
	{⊗}{{\ensuremath{\otimes}}}1
	{⊞}{{\ensuremath{\boxplus}}}1

	{∇}{{\ensuremath{\nabla}}}1
	{√}{{\ensuremath{\sqrt}}}1

	{⬝}{{\ensuremath{\cdot}}}1
	{•}{{\ensuremath{\cdot}}}1
	{∘}{{\ensuremath{\circ}}}1

	%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
	{⁻}{{\ensuremath{^{-}}}}1
	{▸}{{\ensuremath{\blacktriangleright}}}1

	{∧}{{\ensuremath{\wedge}}}1
	{∨}{{\ensuremath{\vee}}}1
	{¬}{{\ensuremath{\neg}}}1
	{⊢}{{\ensuremath{\vdash}}}1

	%{⟨}{{\ensuremath{\left\langle}}}1
	%{⟩}{{\ensuremath{\right\rangle}}}1
	{⟨}{{\ensuremath{\langle}}}1
	{⟩}{{\ensuremath{\rangle}}}1

	{↦}{{\ensuremath{\mapsto}}}1
	{←}{{\ensuremath{\leftarrow}}}1
	{<-}{{\ensuremath{\leftarrow}}}1
	{→}{{\ensuremath{\rightarrow}}}1
	{↔}{{\ensuremath{\leftrightarrow}}}1
	{⇒}{{\ensuremath{\Rightarrow}}}1
	{⟹}{{\ensuremath{\Longrightarrow}}}1
	{⇐}{{\ensuremath{\Leftarrow}}}1
	{⟸}{{\ensuremath{\Longleftarrow}}}1

	{∩}{{\ensuremath{\cap}}}1
	{∪}{{\ensuremath{\cup}}}1
	{⊂}{{\ensuremath{\subseteq}}}1
	{⊆}{{\ensuremath{\subseteq}}}1
	{⊄}{{\ensuremath{\nsubseteq}}}1
	{⊈}{{\ensuremath{\nsubseteq}}}1
	{⊃}{{\ensuremath{\supseteq}}}1
	{⊇}{{\ensuremath{\supseteq}}}1
	{⊅}{{\ensuremath{\nsupseteq}}}1
	{⊉}{{\ensuremath{\nsupseteq}}}1
	{∈}{{\ensuremath{\in}}}1
	{∉}{{\ensuremath{\notin}}}1
	{∋}{{\ensuremath{\ni}}}1
	{∌}{{\ensuremath{\notni}}}1
	{∅}{{\ensuremath{\emptyset}}}1

	{∖}{{\ensuremath{\setminus}}}1
	{†}{{\ensuremath{\dag}}}1

	{ℕ}{{\ensuremath{\mathbb{N}}}}1
	{ℤ}{{\ensuremath{\mathbb{Z}}}}1
	{ℝ}{{\ensuremath{\mathbb{R}}}}1
	{ℚ}{{\ensuremath{\mathbb{Q}}}}1
	{ℂ}{{\ensuremath{\mathbb{C}}}}1
	{⌞}{{\ensuremath{\llcorner}}}1
	{⌟}{{\ensuremath{\lrcorner}}}1
	{⦃}{{\ensuremath{\{\!|}}}1
	{⦄}{{\ensuremath{|\!\}}}}1

	{‖}{{\ensuremath{\|}}}1
	{₁}{{\ensuremath{_1}}}1
	{₂}{{\ensuremath{_2}}}1
	{₃}{{\ensuremath{_3}}}1
	{₄}{{\ensuremath{_4}}}1
	{₅}{{\ensuremath{_5}}}1
	{₆}{{\ensuremath{_6}}}1
	{₇}{{\ensuremath{_7}}}1
	{₈}{{\ensuremath{_8}}}1
	{₉}{{\ensuremath{_9}}}1
	{₀}{{\ensuremath{_0}}}1
	{ᵢ}{{\ensuremath{_i}}}1
	{ⱼ}{{\ensuremath{_j}}}1
	{ₐ}{{\ensuremath{_a}}}1

	{¹}{{\ensuremath{^1}}}1

	{ₙ}{{\ensuremath{_n}}}1
	{ₘ}{{\ensuremath{_m}}}1
	{ₚ}{{\ensuremath{_p}}}1
	{ₖ}{{\ensuremath{_\mathrm{k}}}}1
	{↑}{{\ensuremath{\uparrow}}}1
	{↓}{{\ensuremath{\downarrow}}}1

	{...}{{\ensuremath{\ldots}}}1
	{·}{{\ensuremath{\cdot}}}1

	{▸}{{\ensuremath{\triangleright}}}1

	{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
	{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
	{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
	{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
	{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
	{\$}{{\color{symbolcolor}\$}}1

	{:=}{{\color{symbolcolor}:=}}1
	{=}{{\color{symbolcolor}=}}1
	{<|>}{{\color{symbolcolor}<|>}}1
	{<\$>}{{\color{symbolcolor}<\$>}}1
	{+}{{\color{symbolcolor}+}}1
	{*}{{\color{symbolcolor}*}}1,

	% Comments
	%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
	morecomment=[s][\color{commentcolor}]{/-}{-/},
	morecomment=[l][\itshape \color{commentcolor}]{--},

	% Spaces are not displayed as a special character
	showstringspaces=false,

	% keep spaces
	keepspaces=true,

	% String delimiters
	morestring=[b]",
	morestring=[d],

	% Size of tabulations
	tabsize=3,

	% Enables ASCII chars 128 to 255
	extendedchars=false,

	% Case sensitivity
	sensitive=true,

	% Automatic breaking of long lines
	breaklines=true,
	breakatwhitespace=true,

	% Default style fors listingsred
	basicstyle=\ttfamily\small,

	% Position of captions is bottom
	captionpos=b,

	% Full flexible columns
	columns=[l]fullflexible,


	% Style for (listings') identifiers
	identifierstyle={\ttfamily\color{black}},
	% Note : highlighting of Coq identifiers is done through a new
	% delimiter definition through an lstset at the beginning of the
	% document. Don't know how to do better.

	% Style for declaration keywords
	keywordstyle=[1]{\ttfamily\color{keywordcolor}},

	% Style for sorts
	keywordstyle=[2]{\ttfamily\color{sortcolor}},

	% Style for tactics keywords
	keywordstyle=[3]{\ttfamily\color{tacticcolor}},

	% Style for attributes
	keywordstyle=[4]{\ttfamily\color{attributecolor}},

	% Style for strings
	stringstyle=\ttfamily,

	% Style for comments
	commentstyle={\ttfamily\footnotesize },

}
